MedMCQA : A Large-scale Multi-Subject Multi-Choice Dataset for Medical domain Question Answering

This paper introduces MedMCQA, a new large-scale, Multiple-Choice Question Answering (MCQA) dataset designed to address real-world medical entrance exam questions. More than 194k high-quality AIIMS \& NEET PG entrance exam MCQs covering 2.4k healthcare topics and 21 medical subjects are collected with an average token length of 12.77 and high topical diversity. Each sample contains a question, correct answer(s), and other options which requires a deeper language understanding as it tests the 10+ reasoning abilities of a model across a wide range of medical subjects \& topics. A detailed explanation of the solution, along with the above information, is provided in this study.

==> images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}

